BrickSmart: Leveraging Generative AI to Support Children's Spatial Language Learning in Family Block Play

Block-building activities are crucial for developing children's spatial reasoning and mathematical skills, yet parents often lack the expertise to guide these activities effectively. BrickSmart, a pioneering system, addresses this gap by providing spatial language guidance through a structured three-step process: Discovery & Design, Build & Learn, and Explore & Expand. This system uniquely supports parents in 1) generating personalized block-building instructions, 2) guiding parents to teach spatial language during building and interactive play, and 3) tracking children's learning progress, altogether enhancing children's engagement and cognitive development. In a comparative study involving 12 parent-child pairs children aged 6-8 years) for both experimental and control groups, BrickSmart demonstrated improvements in supportiveness, efficiency, and innovation, with a significant increase in children's use of spatial vocabularies during block play, thereby offering an effective framework for fostering spatial language skills in children.

==> table/tab_dimensions_app.tex <==
\begin{table}[h]
\label{tab:dimensions}
\caption{Eight dimensions of spatial language and the corresponding vocabularies \cite{cannon2007system} used in the BrickSmart system.}
%\vspace{-10pt}
\small % 或者使用 \scriptsize 来获得更小的字体
\begin{tabular}{>{\centering\arraybackslash}m{1cm}m{11cm}}
\toprule
 & \multicolumn{1}{c}{\textbf{Spatial Language Vocabularies}}\\ 
\midrule
\multicolumn{1}{l}{\textbf{1. Spatial Dimensions}} & 
Big/Little, Long/Short, High/Low, Wide/Narrow, Thick/Thin, Skinny/Fat, Deep/Shallow, Full/Empty, Length, Height, Width, Depth, Volume, Capacity, Area.  \\
\midrule
\multicolumn{1}{l}{\textbf{2. Shapes}} & 
Circle, Square, Rectangle, Triangle, Oval, Semicircle, Polygon, Cube, Sphere, Cylinder, Cone. \\
\midrule
\multicolumn{1}{l}{\textbf{3. Locations and Directions}} & 
At, To/From, On/Off, Ahead/Behind, Left/Right, In/Out, Between/Aside, Opposite, Position, Direction, Distance, Path. \\
\midrule
\multicolumn{1}{l}{\makecell[l]{\textbf{4. Orientations and }\\\textbf{\quad Transformations}}} & 
Forward/Backward, Turn left/right, Upward/Downward, Flip, Rotate, Slide, Clockwise/Counterclockwise. \\
\midrule
\multicolumn{1}{l}{\textbf{5. Continuous Amount}} & 
Whole/Part, All/Half/Fraction, A lot/A little, More/Less, Same/Equal. \\
\midrule
\multicolumn{1}{l}{\textbf{6. Deictics}} & 
Here, There, Where, This, That, Which.  \\
\midrule
\multicolumn{1}{l}{\makecell[l]{\textbf{7. Spatial Features and} \\ \textbf{\quad Properties}}} & 
Line, Curve, Edge, Flat, Bent/d, Point, Acute angle, Obtuse angle, Right angle, Vertical, Parallel.\\
\midrule
\multicolumn{1}{l}{\textbf{8. Pattern}} & 
Increase/Decrease, Before/After, Next/Last, First/Last, Order, Repeat, Pattern.  \\
\bottomrule
\end{tabular}
%\vspace{-20pt}
\end{table}



==> table/tab_dimensions_chinese.tex <==
\begin{table}[h]
\label{tab:dimensions}
\caption{Chinese version of eight dimensions of spatial language and the corresponding vocabularies \cite{cannon2007system} used in the BrickSmart system.}
\small % 或者使用 \scriptsize 来获得更小的字体
\begin{tabular}{>{\centering\arraybackslash}m{1cm}m{11cm}}
\toprule
 & \multicolumn{1}{c}{\textbf{空间语言词汇}}\\ 
\midrule
\multicolumn{1}{l}{\textbf{1. 空间维度}} & 
大/小, 长/短, 高/低, 宽/窄, 厚/薄, 粗/细, 深/浅, 满/空, 长度, 高度, 宽度, 深度, 体积, 容积, 面积 \\
\midrule
\multicolumn{1}{l}{\textbf{2. 形状}} & 
圆形, 正方形, 长方形, 三角形, 椭圆形, 半圆, 多边形, 立方体, 球体, 圆柱体, 圆锥体 \\
\midrule
\multicolumn{1}{l}{\textbf{3. 位置和方向}} & 
在, 从/到, 上/下, 前/后, 左/右, 里/外, 中间/旁边, 相对, 位置, 方向, 距离, 路径 \\
\midrule
\multicolumn{1}{l}{\textbf{4. 方向和变换}} & 
向前/后, 向左/右, 向上/下, 翻转, 旋转, 滑动, 顺时针/逆时针\\
\midrule
\multicolumn{1}{l}{\textbf{5. 连续量}} & 
整体/部分, 全部/一半/几分之一, 多数/少数, 更多/少, 相等 \\
\midrule
\multicolumn{1}{l}{\textbf{6. 指示词}} & 
"这里", "那里", "哪里", "这个", "那个", "哪个" \\
\midrule
\multicolumn{1}{l}{\textbf{7. 空间特征和属性}} & 
直线, 曲线, 边缘, 平面, 曲面, 点, 锐角, 钝角, 直角, 垂直, 平行\\
\midrule
\multicolumn{1}{l}{\textbf{8. 模式}} & 
增加/减少, 之前/之后, 下一个/上一个, 第一个/最后一个, 顺序, 重复, 模式 \\
\bottomrule
\end{tabular}

\end{table}

==> table/tab_prompt_chinese.tex <==
\begin{table*}[h!]
\centering
\small
\caption{The original Chinese version of prompts BrickSmart employs across three steps.}
\begin{tabular}{l|p{0.9cm}|p{12.5cm}}
\toprule
\textbf{Steps} & \textbf{Goal} & \textbf{System Prompts}\\ \hline
\multirow{2}{*}{Step 1} & Generate descriptions & 你的任务是孩子讲述的故事和场景分解成几个可描述的3D对象，并依次输出到结构化的字符串列表 object\_list[] 中。
例如，孩子说“大眼睛的猴子在爬树”，则输出字符串列表 object\_list=["猴子，大眼睛，动作是正在爬树", "树"]。
请你仅按照孩子的描述来分解和输出，不要添加额外的信息或者自己的想法。如果孩子描述的内容不够详细，则输出空白字符串列表 object\_list=[]。
现在已经有了初步的列表信息：\{object\_list\}。
你需要根据新的描述或者已有内容，完善和补充列表中的条目。
之前的对话历史如下： \{chat\_history\} \\ \cline{2-3}
& Generate prompts for 3D models & 
You are an expert at crafting text prompts for generating 3D models, specializing in transforming children's imaginative words and narrated diaries into delightful, cartoon-style 3D models. Your prompts should focus on describing a single object rather than a scene, ensuring that the description is suitable for conversion into LEGO models. When rewriting user input, consider the following: The generated 3D model should avoid unnecessary details, should have a suitable center of gravity, and should clearly and independently represent a single entity. The appearance can be slightly enhanced to appeal to the aesthetic preferences of 6-8-year-old children. 
Ensure the model is suitable for construction using only basic LEGO bricks, emphasizing square and rectangular forms. Your output should be a detailed sentence or a list of descriptive words separated by commas, written in English.
\\ \hline
\multirow{3}{*}{Step 2} & Under-standing tutorial images & 根据提供的乐高拼装教程图片，详细分析并描述当前积木搭建任务，输出字符串参数 instruction：
 (1) 图片展示的乐高模型的整体构造和设计特点。
 (2) 识别并描述图片中出现的乐高零件种类及其颜色。
 (3) 指出图片中的拼装步骤，包括任何特别的组装技巧或需要特别注意的细节。
 (4) 使用专业的乐高术语来增加描述的准确性和专业性。
 (5) 确保输出的文字描述准确反映图片内容，语言表达清晰、专业、详细，便于读者理解拼装过程。\\ \cline{2-3}
& Vocabu-lary selection & 你是一个空间语言教师，你的职责是根据任务和学生情况判断该学习的空间语言任务。请根据以下信息： 乐高拼装教程描述 \{instruction\}. 空间语言的8个维度: ...  
用户当前对空间语言的掌握程度是：\{understand\_level\}，代表了8个维度分别的学习进度（以百分比表示）。
判断最适合学习的3个空间语言类别，尽量挑选适合当前积木搭建任务且用户掌握程度不高的类别。
输出长度为3的列表 spatial\_list，每个元素的取值范围为0-7，代表空间语言类别的索引。\\ \cline{2-3}
& Guidance generation & 你是一个家庭引导师，你的职责是帮助家长引导孩子并提升空间语言能力。你需要根据目前乐高搭建教程的步骤，实时为家长生成引导提示。
当前需要学习的空间词汇和对应的阶段包括：
1. 词汇：\{word\_1\}，学习阶段：\{stage\_1\}；
2. 词汇：\{word\_2\}，学习阶段：\{stage\_2\}；
3. 词汇：\{word\_3\}，学习阶段：\{stage\_3\}；
当前乐高搭建的教程为：\{instruction\}，图片中包含俯视图（top view）-为当前步骤要搭建的积木块，和整体视图（whole view）-包含当前任务和之前已搭建好的所有。
请理解当前的搭建任务，在引导搭建孩子的过程中学习以上三个词汇，分别符合对应的学习阶段，为家长生成提示和举例。
示例格式输出：
1. 词汇：圆形，学习阶段：名词解释
提示：可以告诉孩子，圆形是一种没有角的形状，边上的每一点到中心点的距离都是一样的。
示例：在搭建过程中可以找到圆形的积木块，或者积木块上的圆形图案，帮助他们理解。\\ \hline
\multirow{2}{*}{Step 3}& Guidance generation & 你是一个帮助家长与孩子互动的助手，目标是提升孩子的空间语言表达能力。孩子和家长当前使用乐高积木搭建了几个乐高模型，包括：\{objects\}。
你的任务是引导家长和孩子，通过让这些乐高模型“动起来”来描述它们的状态，从而增强孩子对空间概念的理解。家长可以移动搭建好的上述乐高模型，或乐高积木，并让孩子描述这些动作。
请按照以下格式输出互动建议：
词汇：要学习的空间语言词汇, 动态指令例子：给出移动物体的具体方法, 家长引导语示例：提供家长可以使用的引导语, 示例格式输出：
1. 词汇：向左/向右; 动态指令例子：让小人向前走，然后向左转; 家长引导语示例：你看这个可爱的小人，他往前走，然后向左转啦。你能让小人向右转吗？
针对下列 \{num\_words\} 个关键词：\{keywords\}，逐个输出互动建议。\\ \bottomrule
\end{tabular}
\label{tab:ChinesePrompts}
\end{table*}





